Approximating Edit Distance Within Constant Factor in Truly Sub-Quadratic Time

Edit distance is a measure of similarity of two strings based on the minimum number of character insertions, deletions, and substitutions required to transform one string into the other. The edit distance can be computed exactly using a dynamic programming algorithm that runs in quadratic time. Andoni, Krauthgamer, and Onak (2010) gave a nearly linear time algorithm that approximates edit distance within an approximation factor $\text{poly}(\log n)$. In this paper, we provide an algorithm with running time $\tilde{O}(n^{2-2/7})$ that approximates the edit distance within a constant factor.

==> edge-set-pdf.tex <==
 \begin{figure}[ht]
  \centering
  \begin{tikzpicture}[scale=0.3,shorten >=1mm,>=latex]
   \tikzstyle gridlines=[color=black!20,very thin]
       
       \draw[black,dotted] (-23,15) -- (-23,37);
       \draw[black,dotted] (-11,15) -- (-11,37);
       
       \draw[gray!70,thick] (-23,20) rectangle (-11,32);
       
       \draw[black,dotted] (-27,18) -- (-23,18);
       \draw[black,dotted] (-11,29.5) -- (-7,29.5);
       
       %\draw[black,thick,->,dashed] (-27.2,16) -- (-25,18.15);
       %\draw[black,thick,->,dashed] (-25.2,18) -- (-22.8,18);
       \draw[black,thick,->,dashed] (-24.5,16) -- (-22.6,17.3);
       \draw[black,thick,->,dashed] (-23,17) -- (-23,20.2);
       \draw[black,thick,->,dashed] (-23,20) -- (-23,23);
       \draw[black,thick,->,dashed] (-23,22.75) -- (-10.8,29.1);
       \draw[black,thick,->,dashed] (-11,29.1) -- (-11,35.2);
       \draw[black,thick,->,dashed] (-11,34.8) -- (-9,36.4);
       
       
      % \draw[black,color=blue,thick] (-26,15) -- (-23.85,17.15);
       %\draw[black,color=blue,thick] (-24,17) -- (-24,19.15);
       %\draw[black,color=blue,thick] (-24,19) -- (-21.85,19);
       %\draw[black,color=blue,thick] (-22,19) -- (-17.85,23.15);
       %\draw[black,color=blue,thick] (-18,23) -- (-18,24.15);
       %\draw[black,color=blue,thick] (-18,24) -- (-11.8,31);
       %\draw[black,color=blue,thick] (-11.8,31) -- (-10,31);
       
       
       
       \draw [black,thick] plot [smooth,tension=1] coordinates {(-25.5,15) (-24.6,17.5) (-21.5,19)};
       \draw [black,thick] plot [smooth,tension=1] coordinates {(-21.5,19.28) (-20.8,20) (-20.75,20.95)};
       \draw [black,thick] plot [smooth,tension=1] coordinates {(-20.75,21.2) (-19.5,25) (-15.5,27.4)};
       \draw [black,thick] plot [smooth,tension=1] coordinates {(-15.49,27.7) (-14.8,28.3) (-14.3,29.1)};
       \draw [black,thick] plot [smooth,tension=1] coordinates {(-14.3,29.3) (-13.3,30.5) (-11,30.9)};
       \draw [black,thick] plot [smooth,tension=1] coordinates {(-11,31.1) (-10,31.6) (-8.7,32.9)};
       
       
       \node at (-22,17.1)[scale=.8] {$r_{i-1}'$};
       \node at (-24.5,18.5)[scale=.8] {$r_{i-1}$};
       \node at (-23.6,22.9)[scale=.8] {$t_i'$};
       \node at (-21.2,20.4)[scale=.8] {$t_i$};
       \node at (-10.5,28.9)[scale=.8] {$r_i'$};
       \node at (-8.5,30.7)[scale=.8] {$r_i=t_{i+1}$};
       \node at (-12,34.7)[scale=.7] {$t_{i+1}'$};
       \node at (-18,24.8)[scale=.8] {$e$};
       \node at (-23.6,20)[scale=.9] {$s_i$};
       \node at (-10,32.5)[scale=.8] {$s_{i+1}$};
       
       \draw[fill=black] (-23,22.8) circle (.1cm);
       \draw[fill=black] (-23,20) circle (.1cm);
       \draw[fill=black] (-24,18) circle (.1cm);
       \draw[fill=black] (-20.8,20) circle (.1cm);
       \draw[fill=black] (-23,17.1) circle (.1cm);
       \draw[fill=black] (-11,29) circle (.1cm);
       \draw[fill=black] (-11,31.05) circle (.1cm);
       \draw[fill=black] (-11,34.8) circle (.1cm);
       \draw[fill=black] (-11,32) circle (.1cm);
       
      
       %\node at (-17,14)[scale=1] {(b)};
       
       
       


\end{tikzpicture}
\caption{An example of a path $\tau$ (in solid) passing through a certified box $(I,J,\ell/\mu(I))$. The dashed path is an approximation $\tau'$ of $\tau$ in $\widetilde{G}$. The cost of the subpath of $\tau'$ from $s_i$ to $t'_{i}$ is $\ell$, $\cost(e)=3\ell$, and cost of the subpath of $\tau'$ from $r'_i$ to $s_{i+1}$ is $\le \ell$. So the total cost of the subpath of $\tau'$ from $s_i$ to $s_{i+1}$ is $5 \ell$.}
   \label{fig:path}
\end{figure}  
